Comparative analysis of optical character recognition methods for S\'ami texts from the National Library of Norway

Optical Character Recognition (OCR) is crucial to the National Library of Norway's (NLN) digitisation process as it converts scanned documents into machine-readable text. However, for the S\'ami documents in NLN's collection, the OCR accuracy is insufficient. Given that OCR quality affects downstream processes, evaluating and improving OCR for text written in S\'ami languages is necessary to make these resources accessible. To address this need, this work fine-tunes and evaluates three established OCR approaches, Transkribus, Tesseract and TrOCR, for transcribing S\'ami texts from NLN's collection. Our results show that Transkribus and TrOCR outperform Tesseract on this task, while Tesseract achieves superior performance on an out-of-domain dataset. Furthermore, we show that fine-tuning pre-trained models and supplementing manual annotations with machine annotations and synthetic text images can yield accurate OCR for S\'ami languages, even with a moderate amount of manually annotated data.

==> tables/auto_smi_language_distribution.tex <==
\begin{tabular}{lll}
\toprule
\begin{tabular}[c]{@{}l@{}}North \\ Sámi\end{tabular}                    & \begin{tabular}[c]{@{}l@{}}South \\ Sámi\end{tabular}               & \begin{tabular}[c]{@{}l@{}}Lule \\ Sámi\end{tabular}                   \\ \midrule
\begin{tabular}[c]{@{}l@{}}1810 docs \\ 70413 lines\\  83.6 \%\end{tabular} & \begin{tabular}[c]{@{}l@{}}265 docs\\ 7082 lines\\ 8.4 \%\end{tabular} & \begin{tabular}[c]{@{}l@{}}253 docs\\ 6781 lines\\ 8.0 \%\end{tabular} \\ \bottomrule
\end{tabular}

==> tables/auto_smi_language_distribution_new.tex <==
\begin{tabular}{lll}
\toprule
\makecell[l]{North \\ Sámi} & \makecell[l]{South \\ Sámi} & \makecell[l]{Lule \\ Sámi} \\ \midrule
1810 docs   & 265 docs   & 253 docs   \\
70413 lines & 7082 lines & 6781 lines \\
83.6 \%     & 8.4 \%     & 8.0 \% \\
\bottomrule
\end{tabular}

==> tables/character_errors_old.tex <==
\begin{tabular}{@{}c@{}c@{}ccc@{}c@{}ccc@{}c@{}ccc@{}c@{}cc@{}} \toprule \multicolumn{4}{c}{\textbf{Transkribus}} & \multicolumn{4}{c}{\textbf{Tesseract}} & \multicolumn{4}{c}{\textbf{TrOCR}} & \multicolumn{4}{c}{\textbf{Baseline}} \\ \cmidrule(r){1-4}\cmidrule(lr){5-8}\cmidrule(lr){9-12}\cmidrule(lr){13-16} \multicolumn{3}{c}{Error} & \# & \multicolumn{3}{c}{Error} & \# & \multicolumn{3}{c}{Error} & \# & \multicolumn{3}{c}{Error} & \# \\ \cmidrule(r){1-3}\cmidrule(lr){4-4}\cmidrule(lr){5-7}\cmidrule(lr){8-8}\cmidrule(lr){9-11}\cmidrule(lr){12-12}\cmidrule(lr){13-15}\cmidrule(l){16-16} `â' & \(\rightarrow\) & `á' & 16 & `ï' & \(\rightarrow\) & `i' & 24 & `Á' & \(\rightarrow\) & `A' & 9 & `á' & \(\rightarrow\) & `å' & 313 \\ `â' & \(\rightarrow\) & `a' & 14 & `â' & \(\rightarrow\) & `á' & 22 & `' & \(\rightarrow\) & `l' & 7 & `ï' & \(\rightarrow\) & `i' & 137 \\ `Á' & \(\rightarrow\) & `A' & 9 & `đ' & \(\rightarrow\) & `d' & 12 & `Š' & \(\rightarrow\) & `S' & 6 & `â' & \(\rightarrow\) & `å' & 103 \\ `/' & \(\rightarrow\) & ` ' & 9 & `Á' & \(\rightarrow\) & `A' & 10 & `' & \(\rightarrow\) & `i' & 5 & `–' & \(\rightarrow\) & `-' & 75 \\ `đ' & \(\rightarrow\) & `d' & 7 & `' & \(\rightarrow\) & `d' & 8 & `' & \(\rightarrow\) & ` ' & 4 & `š' & \(\rightarrow\) & `s' & 72 \\ `i' & \(\rightarrow\) & `ï' & 7 & `' & \(\rightarrow\) & `á' & 7 & `Č' & \(\rightarrow\) & `C' & 4 & `đ' & \(\rightarrow\) & `d' & 48 \\ `š' & \(\rightarrow\) & `' & 6 & `' & \(\rightarrow\) & `i' & 7 & `á' & \(\rightarrow\) & `å' & 4 & `á' & \(\rightarrow\) & `a' & 46 \\ `ä' & \(\rightarrow\) & `á' & 5 & `s' & \(\rightarrow\) & `S' & 7 & `i' & \(\rightarrow\) & `ï' & 4 & `â' & \(\rightarrow\) & `á' & 30 \\ `ï' & \(\rightarrow\) & `i' & 5 & `â' & \(\rightarrow\) & `å' & 6 & `Å' & \(\rightarrow\) & `A' & 3 & `â' & \(\rightarrow\) & `ä' & 26 \\ `' & \(\rightarrow\) & `-' & 4 & `.' & \(\rightarrow\) & `' & 5 & `š' & \(\rightarrow\) & `s' & 3 & `č' & \(\rightarrow\) & `c' & 26 \\ \bottomrule \end{tabular}

==> tables/characters.tex <==
\begin{tabular}{lllll}
\cellcolor[HTML]{FFE599} \begin{tabular}[c]{@{}l@{}}South\\ Sámi\end{tabular} & \cellcolor[HTML]{9FC5E8}\begin{tabular}[c]{@{}l@{}}North\\ Sámi\end{tabular} & \cellcolor[HTML]{B6D7A8}\begin{tabular}[c]{@{}l@{}}Lule\\ Sámi\end{tabular} & \cellcolor[HTML]{B4A7D6}\begin{tabular}[c]{@{}l@{}}Inari\\ Sámi\end{tabular} & \cellcolor[HTML]{EA9999}\begin{tabular}[c]{@{}l@{}}Skolt\\ Sámi\end{tabular} \\
& \cellcolor[HTML]{9FC5E8}Áá & \cellcolor[HTML]{B6D7A8}Áá & \cellcolor[HTML]{B4A7D6}Áá & \\
& & & \cellcolor[HTML]{B4A7D6}Ââ & \cellcolor[HTML]{EA9999}Ââ \\
& & & \cellcolor[HTML]{B4A7D6}Ää & \cellcolor[HTML]{EA9999}Ää \\
& \cellcolor[HTML]{9FC5E8}Čč & & \cellcolor[HTML]{B4A7D6}Čč & \cellcolor[HTML]{EA9999}Čč \\
 & & & & \cellcolor[HTML]{EA9999}Ʒʒ \\
 & & & & \cellcolor[HTML]{EA9999}Ǯǯ \\
 & \cellcolor[HTML]{9FC5E8}Đđ & & \cellcolor[HTML]{B4A7D6}Đđ & \cellcolor[HTML]{EA9999}Đđ  \\
 & & & & \cellcolor[HTML]{EA9999}Ǧǧ  \\
 & & & & \cellcolor[HTML]{EA9999}Ǥǥ  \\
\cellcolor[HTML]{FFE599}Ïï  & & & &  \\
 &  & &  & \cellcolor[HTML]{EA9999}Ǩǩ  \\
 & \cellcolor[HTML]{9FC5E8}Ŋŋ  & \cellcolor[HTML]{B6D7A8}Ŋŋ & \cellcolor[HTML]{B4A7D6}Ŋŋ   & \cellcolor[HTML]{EA9999}Ŋŋ  \\
 &  & &  & \cellcolor[HTML]{EA9999}Õõ  \\
 & \cellcolor[HTML]{9FC5E8}Šš  & & \cellcolor[HTML]{B4A7D6}Šš  & \cellcolor[HTML]{EA9999}Šš  \\
 & \cellcolor[HTML]{9FC5E8}Ŧŧ  & &  &  \\
 & \cellcolor[HTML]{9FC5E8}Žž  & & \cellcolor[HTML]{B4A7D6}Žž  & \cellcolor[HTML]{EA9999}Žž  \\
\cellcolor[HTML]{FFE599}Öö  &  & &  & \cellcolor[HTML]{EA9999}Öö \\
 & & & & \cellcolor[HTML]{EA9999} ʹʼˈ \\
\end{tabular}

==> tables/characters_new.tex <==

\begin{tabular}{lllll}
\toprule
\makecell{North} & \makecell{South} & \makecell{Lule} & \makecell{Inari} & \makecell{Skolt} \\
\midrule 
\customfont Áá &  & \customfont Áá & \customfont Áá &  \\
 &  &  & \customfont Ââ & \customfont Ââ \\
 &  &  & \customfont Ää & \customfont Ää \\
 & \customfont Ïï &  &  &  \\
 &  &  &  & \customfont Õõ \\
 & \customfont Öö &  &  &  \\
\customfont Čč &  &  & \customfont Čč & \customfont Čč \\
\customfont Đđ &  &  & \customfont Đđ & \customfont Đđ \\
\customfont Ŋŋ &  & \customfont Ŋŋ & \customfont Ŋŋ & \customfont Ŋŋ \\
\customfont Šš &  &  & \customfont Šš & \customfont Šš \\
\customfont Ŧŧ &  &  &  &  \\
\customfont Žž &  &  & \customfont Žž & \customfont Žž \\
 &  &  &  & \customfont Ʒʒ \\
 &  &  &  & \customfont Ǥǥ \\
 &  &  &  & \customfont Ǧǧ \\
 &  &  &  & \customfont Ǩǩ \\
 &  &  &  & \customfont Ǯǯ \\
 &  &  &  & \customfont ʹ \\
 &  &  &  & \customfont ʼ \\
 &  &  &  & \customfont ˈ \\
\bottomrule
\end{tabular}


==> tables/gt_smi_language_distribution.tex <==
\begin{tabular}{|l|l|l|l|}
\hline
                                       & \textbf{train split}                                                                 & \textbf{val split}                                                                 & \textbf{test split}                                                               \\ \hline
\begin{tabular}[c]{@{}l@{}}North \\ Sámi\end{tabular} & \begin{tabular}[c]{@{}l@{}}2.5 docs\\ 37 pages\\ 5871 lines \\ (91.2\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}8 docs\\ 18 pages\\ 1854 lines \\ (90.4\%)\end{tabular} & \begin{tabular}[c]{@{}l@{}}5 docs\\ 5 pages\\ 239 lines \\ (30.2\%)\end{tabular}  \\ \hline
\begin{tabular}[c]{@{}l@{}}Inari \\ Sámi\end{tabular}    & \begin{tabular}[c]{@{}l@{}}2.5 docs\\ 8 pages\\ 280 lines \\ (4.4\%)\end{tabular}    & \begin{tabular}[c]{@{}l@{}}3 docs\\ 3 pages\\ 109 lines \\ (5.3\%)\end{tabular}    & \begin{tabular}[c]{@{}l@{}}5 docs\\ 6 pages\\ 163 lines \\ (20.6\%)\end{tabular}  \\ \hline
\begin{tabular}[c]{@{}l@{}}South \\ Sámi\end{tabular} & \begin{tabular}[c]{@{}l@{}}5 docs\\ 9 pages\\ 208 lines \\ (3.2\%)\end{tabular}      & \begin{tabular}[c]{@{}l@{}}2 docs\\ 2 pages\\ 53 lines \\ (2.6\%)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}5 docs\\ 5 pages \\ 233 lines \\ (29.5\%)\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}Lule \\ Sámi\end{tabular}     & \begin{tabular}[c]{@{}l@{}}2 docs\\ 4 pages\\ 81 lines \\ (1.3\%)\end{tabular}       & \begin{tabular}[c]{@{}l@{}}2 docs\\ 2 pages\\ 36 lines \\ (1.8\%)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}5 docs\\ 5 pages\\ 156 lines \\ (19.7\%)\end{tabular}  \\ \hline
\end{tabular}

==> tables/gt_smi_language_distribution_new.tex <==
\begin{tabular}{llll}
\toprule
& \textbf{train split} & \textbf{val split} & \textbf{test split} \\ \midrule
North & 2.5 docs   & 8 docs     & 5 docs    \\
Sami  & 37 pages   & 18 pages   & 5 pages   \\
      & 5871 lines & 1854 lines & 239 lines \\
      & (91.2\%)   & (90.4\%)   & (30.2\%)  \\[1.5ex]
Inari & 2.5 docs   & 3 docs     & 5 docs    \\
Sámi  & 8 pages    & 3 pages    & 6 pages   \\
      & 280 lines  & 109 lines  & 163 lines \\
      & (4.4\%)    & (5.3\%)    & (20.6\%)  \\[1.5ex]
South & 5 docs     & 2 docs     & 5 docs    \\
Sámi  & 9 pages    & 2 pages    & 5 pages   \\
      & 208 lines  & 53 lines   & 233 lines \\
      & (3.2\%)    & (2.6\%)    & (29.5\%)  \\[1.5ex]
Lule  & 2 docs     & 2 docs     & 5 docs    \\
Sámi  & 4 pages    & 2 pages    & 5 pages   \\
      & 81 lines   & 36 lines   & 156 lines \\
      & (1.3\%)    & (1.8\%)    & (19.7\%)  \\
\bottomrule
\end{tabular}

==> tables/synth_smi_language_distribution.tex <==
\begin{tabular}{rrrr}
\toprule
\makecell{South \\ Sámi} & \makecell{North \\ Sámi} & \makecell{Lule \\ Sámi} & \makecell{Inari \\ Sámi} \\
\midrule
76971 & 76949 & 76970 & 76497 \\
\bottomrule
\end{tabular}

==> tables/valset_cer_wer.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
 & \multicolumn{3}{c}{Transkribus} & \multicolumn{3}{c}{Tesseract} & \multicolumn{3}{c}{TrOCR} \\
 & CER & WER & mean & CER & WER & mean & CER & WER & mean \\
\midrule
\begin{tabular}[c]{@{}l@{}}GT-Sámi (w/o base)\end{tabular} & 1.59 & 5.67 & 3.63 & 5.53 & 24.70 & 15.11 &  &  &  \\\hline
GT-Sámi & 1.28 & 4.34 & 2.81 & 2.05 & 9.84 & 5.95 & 1.98 & 9.29 & 5.64 \\\hline
\begin{tabular}[c]{@{}l@{}}GT-Sámi\\+GT-Nor\end{tabular} & 1.31 & 4.35 & 2.83 & 2.37 & 11.39 & 6.88 & 1.95 & 8.88 & 5.42 \\\hline
\begin{tabular}[c]{@{}l@{}}GT-Sámi\\+Pred-Sámi\end{tabular} & 1.48 & 4.02 & 2.75 & 1.85 & 8.17 & 5.01 & 1.28 & 5.00 & 3.14 \\\hline
\begin{tabular}[c]{@{}l@{}}GT-Sámi\\+GT-Nor\\+Pred-Sámi\end{tabular} & 1.07 & 3.58 & 2.33 & 1.81 & 7.96 & 4.89 & 1.32 & 5.14 & 3.23 \\\hline
\begin{tabular}[c]{@{}l@{}}GT-Sámi \\(synth base)\end{tabular} &  &  &  & 1.78 & 8.78 & 5.28 & 1.15 & 5.04 & 3.09 \\\hline
\begin{tabular}[c]{@{}l@{}}GT-Sámi\\+Pred-Sámi \\(synth base)\end{tabular} &  &  &  &  &  &  & 1.08 & 4.29 & 2.69 \\\hline
\begin{tabular}[c]{@{}l@{}}GT-Sámi\\+GT-Nor\\+Pred-Sámi \\(synth base)\end{tabular} &  &  &  & 1.79 & 7.70 & 4.75 &  &  &  \\
\bottomrule
\end{tabular}
